Evaluating Theory of (an uncertain) Mind: Predicting the Uncertain Beliefs of Others in Conversation Forecasting

Typically, when evaluating Theory of Mind, we consider the beliefs of others to be binary: held or not held. But what if someone is unsure about their own beliefs? How can we quantify this uncertainty? We propose a new suite of tasks, challenging language models (LMs) to model the uncertainty of others in dialogue. We design these tasks around conversation forecasting, wherein an agent forecasts an unobserved outcome to a conversation. Uniquely, we view interlocutors themselves as forecasters, asking an LM to predict the uncertainty of the interlocutors (a probability). We experiment with re-scaling methods, variance reduction strategies, and demographic context, for this regression task, conducting experiments on three dialogue corpora (social, negotiation, task-oriented) with eight LMs. While LMs can explain up to 7% variance in the uncertainty of others, we highlight the difficulty of the tasks and room for future work, especially in practical applications, like anticipating ``false

==> 01_intro_v2.tex <==
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{latex/figures/intro_question.png}
    \caption{Recognizing uncertainty in others can influence AI dialogue strategies, ultimately improving task-success. Here, an AI assistant recognizes user uncertainty and probes to resolve it, eventually increasing user satisfaction. We formalize tasks to assess language models for their ability to recognize uncertainty in other's beliefs -- an aspect of Theory of Mind. We propose new methods to use language models for this regression task, evaluating eight models across three dialogue corpora.}
    \label{fig:intro}
\end{figure}
%
Theory-of-mind and, specifically, false belief prediction is an integral part of planning and decision-making in conversations \citep{ho2022planning}. For instance, an interlocutor recognizing another's false beliefs can offer clarification or explanation. While beliefs are often treated as existing in a binary state (held or not held), there are situations where an interlocutor’s belief is better represented more flexibly (e.g., held, not held, or \textit{unsure}), capturing the uncertainty or more general intensity of the belief. Strangers in a first encounter may be unsure of how they feel about each other and competing stakeholders in a negotiation may be similarly perplexed about each other’s objectives. In task-oriented settings, people may even be unsure of their goals \citep{sicilia2023isabel}, impeding success when this is not considered (e.g., see Figure~\ref{fig:intro}). How we respond in conversation depends not only on our anticipation of another's belief, but also how strongly they hold that belief. Yet, it’s unclear how conversational AI, like language models, represent the uncertainty of others in dialogue.

This paper tackles this issue, proposing new tasks to evaluate ToM capacity in language models, specifically pertaining to uncertainty. To do this, we use conversation forecasting as a tool. Whereas existing forecasting tasks \citep{sokolova-etal-2008-telling, zhang-etal-2018-conversations, sicilia2024deal}, focus on predicting aleatoric factors of uncertainty, which are inherent to the data and independent of perspective, we focus on predicting subjective and individual factors of uncertainty, held by each interlocutor. 

In particular, we ask models to forecast \textit{the uncertainty of others' beliefs} as well as \textit{the uncertainty of others' beliefs about others}.
%We argue how epistemic uncertainty -- a measure from machine learning quantifying model-dependent (subjective) aspects of uncertainty -- can be used to quantify a human or machine interlocutor's false belief continuously, effectively considering the uncertainty of their belief in tandem. We use this insight to propose a new uncertainty-aware notion of false belief ``\textit{False Uncertainty}'' and use it as a central evaluation tool in our tasks.
% While we are more broadly interested in representing all beliefs on a continuous spectrum, we focus on uncertainty because of its existing formal machinery in probability and forecasting theory \cite{} as well as conversation forecasting. The interlocutor’s uncertainty (the forecast) and the ground-truth world state (an outcome probability) can be compared to highlight the subjective (false) aspects of a belief. Indeed, we use this property in \S blah to define our notion of continuous false belief: False Uncertainty. Nonetheless, we also show how more general annotations on the intensity of a belief can implicitly express an interlocutor’s uncertainty about future events. We use this to provide a unified task description that is amenable to many forms of continuous belief annotations \S~\ref{sec:}.
%
% The type of nuanced uncertainty modeling for which we advocate is imperative for effective human-machine communication. Interlocutors capable of modeling others uncertainty and, more importantly, their ``false'' uncertainty can intervene during conversation to prevent miscommunications \citep{nilsenova}. Indeed, measuring the (rather than hard designations of falsity) is an important qualifier: in a simulated experiment based on real data, we show how much can be gained from modeling false uncertainty, in comparison to only ``hard'' predictions about false beliefs: the actual odds of a miscommunication increase drastically as a function of false uncertainty, even if we control for access to an optimal ``hard'' classifier of interlocutor beliefs. Odds 
%
%In initiating this study of subjective and individual factors in conversational uncertainty modeling, we face two main challenges: (i) how can we precisely capture the subjectivity of an individual's certainty, mathematically and algorithmically; (ii) how can we make use of available conversational data, which rarely comes with \textit{any} interlocutor annotations about mental states -- let alone certainty; and (iii) how can we properly calibrate human \textit{expressions} of certainty to working probabilities. We tackle these problems throughout this paper, offering a collection of principle contributions:
Conversational agents capable of measuring an interlocutors beliefs (or false beliefs) can directly use this ToM capability to inform dialogue strategy. Indeed, in human-human interactions, the accuracy of interlocutor ToM directly influences dialogue behaviors \citep{bara-etal-2021-mindcraft}. For many types of beliefs, like emotions, uncertainty is an important correlate of accuracy \citep{troiano2021emotion}, providing a basis for intervening dialogue acts that can subsequently improve ToM and eventual task-success \cite{nilsenova2001uncertainty}. Recall, Figure~\ref{fig:intro} shows an example of this.

To formalize belief uncertainty, we build on a traditional statistical view, where uncertainty is measured via probability \citep{brocker2009reliability}, granting us an established framework to design our tasks. Belief uncertainty can be measured on a ternary scale (yes, no, maybe) or more general spectrum (e.g., a Likert scale) and we discuss some strategies to calibrate these human annotations to real-world probabilities. Meanwhile, to capture differences in interlocutor perspective, we disentangle this probabilistic notion into two components -- the epistemic (subjective) and the aleatoric (ground-truth) -- common to modern studies of uncertainty in machine learning \citep{hullermeier2021aleatoric}. Interestingly, our formal setup defines a series of regression tasks, allowing us to explore the relatively unexplored area of continuous inference with language models \citep{vacareanu2024words}. In this context, we study the interaction between traditional methodologies (e.g., bagging) and recent advances (e.g., self-consistent chain-of-thought, \citealp{wangself}) for the first time. 
% on a spectrum have more information to inform their dialogue strategy. Indeed, modeling uncertainty is an important aspect of preventing miscommunications, providing a basis for intervening dialogue acts \cite{nilsenova2001uncertainty}. Continuous modeling not only signals \textit{when} to intervene, but \textit{how}. For instance, telling Bob (Figure~\ref{fig:intro}) that Alice “isn't happy with his offer” is not a socially acceptable intervention for a language model. Bob may well respond with ``I never thought she was!'' Instead, suggesting “she didn’t like the offer as much as you think” conveys her true beliefs (relative to his). Interventions like this, which account for uncertainty, can mitigate the unwanted consequences of miscommunications.

In initiating this study of uncertainty-aware ToM evaluation in language models, we offer a few contributions:
\begin{enumerate}[nolistsep]
    \item we formalize ``false uncertainty'' -- a concept akin to false belief -- and connect it to Theory of Mind and forecasting (\S~\ref{sec:tom}), using this to motivate a new task suite (\S~\ref{sec:task_desc});
    % \item we design a new outcome formulation in conversation uncertainty forecasting (\S~\ref{sec:}), which implicitly extracts calibrated annotations about uncertainty from existing corpora;
    \item we propose new methods to forecast others' uncertainty with language models (\S~\ref{sec:meth}), studying ways to use language models for regression and calibrate probability estimates with continuous labels (rather than discrete);
    \item we study how interlocutor demographics, goals, and other conversation context influences the ability of a language model at uncertainty-aware ToM (\S~\ref{sec:exp}).
\end{enumerate}
From experiments (\S~\ref{sec:exp}) across three corpora (social, negotiation, and task-oriented) and eight models, our findings suggest that, language models are able to explain some of the variance in others' uncertainty (up to 7.5\%), with the help of our methods. Yet, we also observe the difficulty of this task, even for humans. We point to areas for future work, including both applications and methodology (\S~\ref{sec:concl}), making code for tasks/evaluation open-source to promote such work.
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{example-image-b}
%     \caption{Anticipating the beliefs of other interlocutors is an important part of conversations, but even optimal ``hard'' classifiers miss out on information. Here, we show regression analysis of a controlled experiment using real conversation data (see \S~\ref{blah:}). The odds of a miscommunication (false belief) increase as a function of false uncertainty, even if we control for access to optimal ``hard'' classifiers of each interlocutor's belief.}
%     \label{fig:enter-label}
% \end{figure}

==> 02_background.tex <==
We focus on the setup of \citet{sicilia2024deal} where an agent observes a conversation and is asked to express their uncertainty about a potential outcome for this conversation; e.g., ``\textit{How much does Speaker A like Speaker B?}'' or ``\textit{Will the negotiation result in a deal?}'' As implied, the conversation is just a partial window into the true (or, eventual) ground-truth. Hidden information, such as future events or mental states, creates an inherent randomness about reality, which may not be fully determined by the available evidence. In this context, we assume a (human) agent forms a mental model capturing their uncertainty about the outcome -- a ``forecast'' about whether the outcome will occur. 
% In the wild, humans manage this kind of uncertainty all the time, meanwhile, conversation forecasting offers a controlled setting to study this skill. 
\subsection{Comparing Forecasts with Ground-Truth}
Given a (potentially partial) conversation and any accompanying evidence about the situation (e.g., interlocutor context), the forecasting agent expresses their uncertainty $P$ about the outcome of interest. For now, we assume $P$ is a probability estimate, but later allow other expressions of uncertainty (\S~\ref{sec:humans}). The forecast $P$ is evaluated by Brier score:
\begin{equation}
    \mathrm{BS} = (P - O)^2
\end{equation}
where $O$ is a binary indicator of the outcome (e.g., 1 if a deal occurs, 0 else). Forecasters with accurate uncertainty estimates (agreeing exactly with the distribution of $O$) will have a lower Brier score than other, less accurate forecasters. Brier score also ranks sub-optimal forecasts with consideration of both calibration and variance \citep{brocker2009reliability}. 
\subsection{The Missing Building Blocks for ToM}
\label{sec:tom}
We observe that Brier score, alone, does not capture the full story about an agent's uncertainty $P$. Indeed, the Brier score measures two individual aspects of uncertainty:
\begin{equation}
  \mathbf{E}[\mathrm{BS}] =  \underbrace{\textbf{Var}[O]}_{\text{aleatoric uncertainty}} + \underbrace{\mathbf{E}[(P - p)^2]}_{\text{epistemic uncertainty}}
\end{equation}
where $p$ is the probability $O=1$.
While the outcome variance captures the inherent randomness of the forecasting task, the latter quantifies the forecaster's excess errors that should not be attributed to this randomness. These model-specific aspects of error make up the \textbf{epistemic uncertainty} \citep{lahlou2022deup, hullermeier2021aleatoric}.
\paragraph{Integrating ToM in Forecasting} 
Uniquely, we consider the epistemic uncertainty of human interlocutors (treated as forecasters) in a conversation. This dual interpretation captures the individual aspects of an interlocutor's uncertainty by comparing
%comparing their forecasts to the (shared) ground-truth. 
% Precisely, it compares 
their forecast to ground-truth.
%quantifying the variance of the forecast around the true outcome probability $p$. In this way, it measures only 
Precisely, it measures the fluctuations in uncertainty caused by the interlocutor themselves -- their knowledge, perceptions, and biases -- rather than those (fluctuations) which may be attributed to changes in ground-truth. Based on the epistemic uncertainty, we define an interlocutor's \textbf{false uncertainty} as:
\begin{equation}
    \mathrm{FUn} = P - p.
\end{equation}
False uncertainty similarly captures subjective fluctuations, but preserves the direction of this subjectivity, distinguishing between positive (over-confident) or negative (under-confident) forms of uncertainty. Quantifying false uncertainty will be the primary motivation for our task design. While works have focused on improving the quality of a forecast (the Brier score), ours is first to propose quantification of other interlocutors' uncertainty.
\paragraph{Other ToM Works}
ToM is often evaluated (in language models) using question-answering \citep{nematzadeh-etal-2018-evaluating, le-etal-2019-revisiting, sap-etal-2022-neural}; which, for instance, mimics common ToM evaluations from psychology, like the Sally-Anne test. Other proposals study machine ToM in situated and collaborative environments \citep{bara-etal-2021-mindcraft, ma-etal-2023-towards-holistic, li-etal-2023-theory}, focus on higher-order ToM \citep{wu-etal-2023-hi}, or consider ToM beyond (more common) belief/false belief anticipation \citep{van-duijn-etal-2023-theory}. Inference-time methods to improve ToM in language models have also been studied \citep{takmaz-etal-2023-speaking, sclar-etal-2023-minding}. Yet, whenever beliefs are involved, they are typically assumed to held or not held. Our forecasting setting is the first to consider anticipation of beliefs/false beliefs with an emphasis on the uncertainty of these beliefs.  
\paragraph{ToM Criteria} 
% A limitation of conversation forecasting on naturally occurring dialogue corpora is the fact that our natural setting foregoes control. Indeed, the uncertainty quantification tasks we propose next do not control for experimental factors like spurious correlations and information-asymmetry, which can be important when evaluating language models \citep{kim-etal-2023-fantom, shapira-etal-2024-clever} to meet criterion for ToM evaluation suggested by \citet{quesque2020theory}. Thus, with the current data, missing factors should be considered before interpreting our tasks as describing ToM ability in a language model. Applying the same tasks with controlled data can lessen these concerns, but we leave this for future work. 
\citet{quesque2020theory} suggest ToM evaluations should require representation of a mental state (the other's) that differs from one's own (\textit{non-merging criterion}) and ensure task-success cannot be based on lower-level processes (\textit{mentalizing criterion}). Language models do not have mental states, so non-merging is achieved by information-asymmetry \citep{kim-etal-2023-fantom}, which forces the model to predict distinct (non-merged) perspectives. In forecasting, this distinction lies in the interlocutor uncertainty $P$ and ground-truth $p$, whenever $P \neq p$. As for \textit{mentalizing}, this criterion is undermined by spurious correlation, to which models are susceptible \citep{kim-etal-2023-fantom, shapira-etal-2024-clever}. Our current, natural conversation corpora (\S~\ref{sec:data}) do not necessarily prevent this risk. Albeit, it has been suggested socially situated tasks (like ours) can alleviate risk \citep{ma2023tomchallenges}. Using our tasks with controlled data can further lessen risk, which we leave as future work.

==> 02_tasks.tex <==
\subsection{Human Expressions of Uncertainty}
\label{sec:humans}
As we are (uniquely) interested in humans as conversation forecasters, probability annotations are not necessarily the most effective way to elicit uncertainty or intensity of belief. Indeed, most of the corpora we study (\S~\ref{sec:data}) annotates belief intensity on a Likert scale; e.g., ``on a scale from 1 to 10, how much do you think Speaker B likes you.'' We focus on probability estimates because these can be compared to ground-truth world states; i.e., whether B actually ``likes,'' to enforce non-merging (\S~\ref{sec:tom}). Without ``the world'' or ``reality'' as reference, we have no way to define subjective, or false, uncertainty. Thus, we map human expressions to probability estimates to enable comparison.
\paragraph{Calibration Strategy: ``More Than Chance''}
Mapping verbal or quasi-continuous expressions of belief uncertainty to probabilities is a calibration problem; e.g., it has been approached for language models using scaling \citep{tian2023just}. In this work, we enable calibration by making a slight semantic change to the outcome of interest. Instead of studying ``whether Speaker B likes Speaker A'' we study ``whether Speaker B likes Speaker A more than would occur by chance.'' This alteration ties belief intensity annotations to a ground-truth outcome that is observable in data. Precisely, following the colloquial meaning of ``more than chance'' in the statistics literature, the ground-truth probability is defined by a $p$-value for the magnitude of the belief, computed from the data. In turn, appending ``more than chance'' defines both ground-truth outcome probabilities and an appropriate calibration function for human expressions of intensity.  We provide details in \S~\ref{sec:extreme}.
\subsection{Uncertainty Quantification (UQ) Tasks}
\label{sec:task_desc}
% We outline three aspects of subjective uncertainty about conversation studied in this work. We discuss how these tasks build to study the conversational skill of False Uncertainty Prediction.
% \paragraph{Introspective Uncertainty (IUQ)} An agent making forecasts about a conversation may be able to model it's own epistemic uncertainty ($\mathrm{EU}$). Practically speaking, this gives the agent a signal about it's biased perception of the world and others, disentangling the subjective aspects of it's uncertainty from ground-truth, and therefore, highlighting its false beliefs. Humans correct themselves all the time (usually when prompted), but we focus on whether modern, machine agents (language models) can represent their epistemic uncertainty about a conversation. Given an agent's forecast $P$ and an estimate $u$ of its epistemic uncertainty $\mathrm{EU}(P)$, we evaluate whether $u \approx \mathrm{EU}$ using metrics from regression: Pearson (linear) correlation, Spearman (rank) correlation, error, and explained variance. Notably, the concept of modeling epistemic uncertainty is not new \citep{deup}, but as we position this task in the context of a conversation, it is important to distinguish between modeling one's own subjective uncertainties (introspection) and modeling the uncertainties of others (Theory of Mind).
\paragraph{1st-Order ToM Uncertainty (1TUQ)} To quantify false uncertainty, one first needs to quantify an interlocutor's base uncertainty about their belief (i.e., the forecast $P$). Aptly, our first task evaluates a language model's ability to quantify the base uncertainty of others. For instance, suppose an interlocutor $\mathrm{A}$ expresses their uncertainty about ``whether $\mathrm{A}$ is happy'' and this is calibrated to a probability forecast $P$.\footnote{Recall, belief intensity needs calibration to a world outcome to make sense as a probability; e.g., ``A tells friends about happiness.'' We use an outcome observable in the data, i.e. ``whether A is happier than would occur by chance.''} The language model's task is to make a prediction $\hat{P}$ about the uncertainty of $\mathrm{A}$'s belief. We evaluate this prediction using regression metrics; e.g., the correlation between $P$ and $\hat{P}$, the absolute error, and the explained variance.
\paragraph{2nd-Order ToM Uncertainty (2TUQ)} Besides their own beliefs, interlocutors also hold uncertainty about the beliefs of others. 
%Of course, in some cases, ``false'' uncertainty prediction entails predicting an interlocutor's false uncertainty about another interlocutor's beliefs, and therefore, predicting the uncertainty of an interlocutor's beliefs about other interlocutors' beliefs. 
For instance, an interlocutor $\mathrm{A}$ can express their uncertainty about ``whether interlocutor $\mathrm{C}$ likes $\mathrm{A}$''. Then, TUQ tasks the language model with quantifying the uncertainty of $\mathrm{A}$ about $\mathrm{C}$'s belief. Similar to the first-order task, we evaluate a language model's prediction by comparing it to $\mathrm{A}$'s true uncertainty.
\paragraph{False Uncertainty (FUnQ)} Finally, we ask language models to directly quantify an interlocutor's false uncertainty. In essence, this requires them to quantify both the interlocutor's uncertainty about a belief as well as the ground-truth probability that the belief is true (the outcome probability $p$). For instance, $P$ may be a forecast about ``whether interlocutor $\mathrm{C}$ likes $\mathrm{A}$'' and $p$ may be the ground-truth probability that ``$\mathrm{C}$ likes $\mathrm{A}$.'' The language model is tasked with quantifying $\mathrm{FUn} = P - p$, and we evaluate this estimation using regression metrics.
%\subsection{Designing Outcomes for Existing Data}
%Unfortunately, available dialogue data typically has (at most) ground-truth annotations on the magnitude/intensity for an interlocutor's belief, rather than their uncertainty. For instance, interlocutors may signal ``how happy they are'' rather than ``how certain they are'' about their emotion. Interestingly, existing studies on (affective) annotations demonstrate high correlation between intensity and certainty \citep{wassa}. Motivated by this, we considered situations where these two mental states are intimately related, designing a new outcome formulation within the conversation forecasting paradigm. Our formulation modifies the outcome of interest to \textit{induce} expressions of interlocutor certainty from existing annotations about magnitude. This solves a data-availability issue as well as a calibration issue (i.e., how do we calibrate annotator expressions of uncertainty to ground-truth world probabilities).
\subsection{Corpora and Basic Prompts}
\label{sec:data}
\paragraph{CaSiNo} is a corpus of negotiations about camp-resource allocation \citep{chawla2021casino}. Interlocutors barter over available resources, such as fire-wood and water, based on (assigned) resource preferences. Performance-based monetary incentives stimulate competitive behaviors. Interlocutors indicate their satisfaction with the final deal on a 5-point scale. For an interlocutor $\mathrm{A}$, we ask language models to predict ``how certain $\mathrm{A}$ is that they are more satisfied than would occur by chance.'' Precise details are in \S~\ref{sec:prompts}. This formulation allows us to evaluate language models for 1st Order ToM uncertainty quantification (1TUQ). The average number of tokens in a conversation is 320.
\paragraph{CANDOR} is a corpus of spoken conversations between strangers, conducted over video communication platform \citep{reece2023candor}. Conversations are social in nature with minimum time constraints and an assigned goal of ``getting to know each other.'' Exit interviews (conducted privately) ask interlocutors to quantify how much they like each other on a 7-point scale, as well as how much they \textit{think} their conversation partner likes them. For two interlocutors $\mathrm{A}$ and $\mathrm{B}$, we ask language models to predict ``how certain is $\mathrm{B}$ that they like $\mathrm{A}$ more than would occur by chance.'' As with CaSiNo, this lets us evaluate language models at the first-order task (1TUQ). Because of the available data, we also ask language models to predict ``how certain is $\mathrm{A}$ that $\mathrm{B}$ likes $\mathrm{A}$ more than would occur by chance.'' As we discuss in \S~\ref{sec:meth}, this lets us evaluate models at the second-order task (2TUQ) and False Uncertainty Quantification (FUnQ). The average token-count is 11K, but we only show models the first 5K.
\paragraph{MultiWOZ} is a task-oriented Wizard-of-Oz corpus wherein one human plays the role of a conversational booking system (for hotels, restaurants, etc.) and the other plays as user \citep{eric-etal-2020-multiwoz}. Additional annotations \citep{sun2021simulating} designate perceived satisfaction of the user by crowd-workers on a 5-point scale. This annotation is less organic than previous datasets, but it can be considered a representative proxy, capturing how annotators might feel if they were in the user's position. As such, we ask language models to predict ``how certain the user is that they are more satisfied than would occur by chance'' using the average crowd-worker annotation as ground-truth. This allow us to evaluate 1TUQ. The average token-count is 460.
% \subsection{Proxy Evaluation Strategy and Corpora}
% Testing each ToM UQ task requires substantial annotations; e.g., about ground-truth probabilities for both outcome and forecaster. Specifically, these are used to compute $\mathrm{EU}$ which is needed for evaluation in each task. Fortunately, we can motivate a reasonable proxy for $\mathrm{EU}$ that only requires observations of the outcomes $O$, which are often easier to obtain in practice. For instance, this lets us conduct proxy evaluation on the \textbf{P4SG corpora.
% \paragraph{Proxy Definition}
% We consider the Brier score $\mathrm{BS}$ as a proxy to stand-in for $\mathrm{EU}$ when some annotations are not available. Indeed, Brier score is a reasonable choice because (i) for IUQ and 1TUQ, it can be estimated with access to (only) outcome observations $O$ and (ii) $\mathrm{BS}$ is (linearly) correlated with $\mathrm{EU}$ in many scenarios:
% % \footnote{By law of total co-variance, and fact $\mathbf{E}[\mathrm{EU} \mid E] = \mathrm{EU}$, we have $\mathbf{cor}(\mathrm{BS}, \mathrm{EU}) = c \cdot \mathbf{cor}(\mathbf{E}[\mathrm{BS} \mid E], \mathrm{EU}) \ \exists c \in [0,1]$. Then, with Eq.~\eqref{eqn:}, we can expand the latter correlation.}
% \begin{equation}
%     \mathbf{cor}(\mathrm{BS}, \mathrm{EU}) \propto \tfrac{k}{k + \mathbf{Var}[V]}
% \end{equation}
% where $V = \mathbf{Var}[O]$ for a fixed conversation and $k$ is a constant independent of $\mathrm{AU}$. So, when the variance of $V$ across the dataset is small, the correlation grows. This will be the case, for instance, when interlocutors have consistently high or consistently low certainty. This means $\mathrm{BS}$ is a metric which often correlates with the evaluation metric for 1TUQ, and requires potentially fewer annotations. For IUQ and 2TUQ, $\mathrm{BS}$ is only a good proxy if correlation (and other metric evaluation) is transitive: $\mathbf{cor}(u, \mathrm{BS})$ and $\mathbf{cor}(\mathrm{BS}, \mathrm{EU})$ implies $\mathbf{cor}(u, \mathrm{EU})$. This is not true for general random variables but, taking into account the specifics of our problem, it turns out that this can be a realistic presumption. Ultimately, we discuss this topic in mathematical detail in \S~\ref{sec:} and conduct experiments to validate this proxy suggestion in \S~\ref{sec:}. 
% % \paragraph{Approximate Transitivity} Intuitively, the aforementioned idea of ``transitivity'' of linear similarity stems from the transitivity of deterministic linear relationships: if $y = mx + b$ and $z = ky + c$, then $z = kmx + (kb + x)$ shows $x$ and $z$ are also linear. Albeit, studying $u$ and $\mathrm{EU}$ does introduce some new variation arising from the randomness of the data. To account for this variation, we can use a common ``pseudo triangle inequality'' for correlations \citep{many}. Specified to our setting, it states: 
% % \begin{equation}
% %     \lvert \mathbf{cor}(u, \mathrm{EU}) - ab \rvert \leq \sqrt{(1-a)^2(1-b)^2}
% % \end{equation}
% % where $a = \mathbf{cor}(u, \mathrm{BS})$ and $b = \mathbf{cor}(\mathrm{BS}, \mathrm{EU})$. As alluded, the principle takeaway is that $\mathbf{cor}(u, \mathrm{BS})$ is an effective proxy for $\mathbf{cor}(u, \mathrm{EU})$ whenever $\mathrm{BS}$ and $\mathrm{EU}$ are correlated. Indeed, as $b \to 1$, the bound tends to zero and $\mathbf{cor}(u, \mathrm{EU}) \approx \mathbf{cor}(u, \mathrm{BS})$. Otherwise, the proxy error scales inversely to the size of $b$, so it can still be (noisily) informative.
% % \subsection{``Downstream'' Behavior Modification}
% % \textcolor{red}{Here we will describe a downstream intervention task based on the uncertainty quantification. If we use a threshold to decide when to intervene, how often can we prevent false beliefs (and their associated errors).}
% \paragraph{Proxy Corpora} We use the same outcomes for \textbf{CaSiNo} and \textbf{CANDOR} in order to validate our proxy evaluation strategy. For these, we show how the proxy can be used with all of the ToM UQ tasks that are originally supported by \textbf{CaSiNo} and \textbf{CANDOR}. We also use the \textbf{DSG} corpora to illustrate how our proxy evaluation can be translated to new outcomes. In particular, we consider the typical future-event outcome ``whether a donation will occur'' and use the Brier score to study IUQ by language models.

==> 03_methods.tex <==
\subsection{Forecasting the Uncertainty of Beliefs}
\label{sec:belief_pred}
Direct Forecasting (\texttt{DF}, \citealp{sicilia2024deal}) is a good ``out-of-the-box'' method for uncertainty-aware conversation forecasting with language models. Adapted to our belief anticipation problem, we prompt the language model to express its predicted uncertainty for the interlocutor on a 10-point scale. We parse the prediction directly from the model's sampled completion and divide by 10 to get an estimate $\hat{P}$ for the interlocutor's true forecast $P$. In general, we use the Chain of Thought (CoT) strategy proposed by \citet{kojima2022large}, asking the model to approach the prediction ``step-by-step.''
\subsubsection{Post-Hoc Scaling}
\label{sec:scaling}
Post-hoc scaling (calibration) tends to improve direct forecasts \citep{tian2023just, sicilia2024deal}, requiring only a small amount of data. 
% We use $n=100$ in our experiments. 
Notably, our ToM tasks work with continuous uncertainty annotations in place of traditional, discrete outcome annotations. We propose new scaling methods to accommodate our data.
\paragraph{Platt Scaling (PS)} One option is to assume the relationship between the true uncertainty $P$ and the predicted uncertainty $\hat{P}$ is linear in the logits; e.g., this is common in soft classification \citep{platt1999probabilistic}. In our new setting,
\begin{equation}
\label{eqn:platt}
    \mathrm{logit}(P) \approx \alpha \cdot \mathrm{logit}(\hat{P}) + \beta.
\end{equation}
The new (re-scaled) forecast is:
\begin{equation}
    \hat{P}_{\mathrm{PS}} = \mathrm{expit} \big (\alpha \cdot \mathrm{logit}(\hat{P}) + \beta \big )
\end{equation}
where $\alpha$, $\beta$ are the OLS estimates of Eq.~\eqref{eqn:platt}.
\paragraph{Linear Scaling (LS)} We also suggest linear scaling, which instead learns a direct linear map:
\begin{equation}
    \hat{P}_{\mathrm{LS}} = \mathrm{clip}(\alpha \cdot \hat{P} + \beta, 0, 1).
\end{equation}
% \begin{equation}
%     P \approx \alpha \cdot \hat{P} + \beta.
% \end{equation}
% Again, $\alpha$ and $\beta$ are learned by minimizing MSE.
% Although logit-linear scaling is more common with soft classifiers, our unique data and tasks allows us to explore linear scaling relationships for the first time. 
\subsubsection{Fine-Tuning a Regression Head}
Fine-tuning a classification head on a language model's latent features 
%or fine-tuning the full language model's token distribution \citep{sicilia} 
can help forecasting performance in soft classification \citep{kadavath2022language}. Again, since our annotations are continuous, we slightly modify this, replacing the classification head with a regression head. Specifically, using the same prompt as \texttt{DF}, the language model encodes latent features $\mathbf{x}$ and inference is conducted as:
\begin{equation}
    \hat{P}_{\mathrm{FT}} = f_\theta(\mathbf{x})
\end{equation}
where $f_\theta$ is the regression head. We test a linear regression head (\texttt{FT L}), a 2-layer ReLU-network head (\texttt{FT NN}), and a random forest head (\texttt{FT RF}). Details are in \S~\ref{sec:optim}.
\subsubsection{Bias and Variance}
\label{sec:b_and_v}
Classically, for a fixed probability $P$, the MSE of a corresponding estimate $\hat{P}$ can be decomposed:
\begin{equation}
    \mathbf{E}[(P - \hat{P})^2] = \textbf{Var}[\hat{P}] + \textbf{Bias}^2(P, \hat{P})
\end{equation}
where $\textbf{Bias}(P, \hat{P}) = \mathbf{E}[\hat{P}] - P$. This points to two possible ways we can reduce error, discussed next.
\paragraph{Bagging} or Bootstrap Aggregating trains many models on random samples from the same data and averages the predictions of all the models. For instance, this is how random forests (\texttt{RF}) are trained \citep{breiman2001random}. It is a known variance reduction strategy, and is why we explore \texttt{RF} as a regression head.
Another strategy we can take, with language models, is to ``bag'' the Chain-of-Thought (CoT) inferences generated when we ask a model to think ``step-by-step''; i.e., we suggest re-sampling the direct forecasts produced by this CoT prompt many times ($n=10$) and averaging these to make an inference. The changes in sampling distribution triggered by each new explanation make this distinct from greedy decoding (see Table~\ref{tab:mce_v_temp}). This strategy is akin to traditional bagging, except we re-sample model explanations, instead of training data. We call this approach a ``Bag of Thoughts'' (\textbf{BoT}). Our strategy is also similar to, yet distinct from, self-consistent decoding in classification \citep{wangself}, where a majority vote is used to aggregate multiple CoT inferences. With majority votes, variance reduction is not necessarily a plausible motivation, since the bias-variance trade-off is not well defined in classification \citep{brown2024bias} and reducing variance can actually increase errors \citep{james2003variance}. Ours is the first work to connect CoT aggregation to variance reduction. Indeed, like bagging, one can show BoT lowers the variance of the direct forecasts (i.e., compared to $n=1$) using basic properties of variance. 
% For scaling, BoT lowers variance of the regression feature, rather than the prediction itself; we still expect this to help by increasing the signal-to-noise ratio. 
% Although CoT aggregation is distinct from greedy decoding (it changes the sampling distribution), we do provide comparison in Table~\ref{tab:mce_v_temp} for completeness.
% this is distinct from setting temperature to 0, since the language models \textit{explain while giving their answer}. That is, we sample these explanations as well, changing the conditional distribution of each inference. For completeness, we compare to greedy sampling in Table~\ref{tab:mce_v_temp}.
% As we are aware, ours is the first work to explore these strategies in regression with language models. 
\paragraph{Demographic Data} provides important background information about the interlocutor in question. Particularly, we consider the age, sex, race, and education of the interlocutor. We hypothesize these characteristics reduce prediction bias because they add situational context, an important aspect of Theory of Mind \citep{ma-etal-2023-towards-holistic}. Moreover, language models are known to inherent and propagate certain social biases \citep{gallegos2023bias} and improved context representations -- such as those achieved by making demographics clear -- can be an effective means to mitigate the biases in generative inference \citep{sicilia2023learning}.
\subsection{Forecasting False Uncertainty}
A straightforward way to predict false uncertainty is to have the model shift perspectives across two inference steps. For instance, in CANDOR, we predict $\mathrm{A}$'s uncertainty about ``whether $\mathrm{C}$ likes $\mathrm{A}$...'' and then predict the ground-truth probability that ``$\mathrm{C}$ likes $\mathrm{A}$...'', shifting perspectives from $\mathrm{A}$ to the outside world. Denoting these $\hat{P}$ and $\hat{p}$, respectively, the following estimates false uncertainty:
\begin{equation}
    \hat{\mathrm{FUn}} = \hat{P} - \hat{p}.
\end{equation}
The same strategies discussed in \S~\ref{sec:belief_pred} can be used to make the individual components of this inference, learning $\hat{p}$ and $\hat{P}$, separately. Alternatively, one can estimate $\hat{\mathrm{FUn}}$ directly. This makes the most sense in the fine-tuning setting, where both latent representations (from the $\hat{p}$ and the $\hat{P}$ prompt) can interact in a (non-linear) regression head to improve inference. We append \texttt{J} (joint learning) to denote this strategy.
% \begin{table}[]
% \centering\small
% \begin{tabular}{lllll}
% && \multicolumn{3}{c}{Tasks} \\\cmidrule(lr){3-5}
% \multicolumn{2}{c}{Data}          & 1TUQ & 2TUQ & FUnQ   \\\cmidrule(lr){1-2}
% \textbf{CANDOR}    & EV      & \checkmark & \checkmark  & \checkmark \\
%           & O       & \xmark   & \xmark    & \xmark    \\\hline
% \textbf{CaSiNo}    & EV      & \checkmark   & \xmark    & \xmark \\
%           & O       & \xmark   & \xmark    & \xmark     \\\hline
% \textbf{MultiWOZ}    & EV      & \checkmark   & \xmark    & \xmark \\
%           & O       & \xmark   & \xmark    & \xmark     \\\hline
% \end{tabular}
% \caption{Forecasting extreme values (EV) instead of typical outcomes (O) lets us implicitly capture uncertainty annotations without changing the task semantics much. Tasks with supported annotations are shown above.}
% \end{table}

==> 04_experiments.tex <==
\begin{table}[]
\centering\small
\begin{tabular}{llllll}
   \texttt{method} & \texttt{xl}    & MAE     & $R^2$     & $\min$ & $\max$ \\\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-6}
\texttt{DF}  & \xmark    & 44.9 & -370 & -620  & -110   \\
\texttt{DF (LS)}& \xmark & \textbf{22.2} & \textbf{1.5} & -4.1  & 7.5  \\
\texttt{DF (PS)}& \xmark & 31.9 & -180 & -740  & -1.8  \\
\texttt{FT (L)} & \xmark &  22.5    &  -1.0     & -2.3     & 1.1  \\\hline
\texttt{DF (LS)}& \checkmark  &   22.1    &  \textbf{2.1} & -5.3  & 12.5 \\ 
\texttt{FT (L)} &\checkmark  &  22.2    &  0.1 & -5.1  & 3.7 \\
\texttt{FT (NN)} &\checkmark  &  22.3    &  -9.2 & -30.5  & 5.4 \\   
\texttt{FT (RF)} &\checkmark  &  \textbf{21.9}    &  1.3 & -5.4  & 7.6 \\
% \hline
% \texttt{H \ (LS)} & \xmark  &  21.9    &  2.7 & -1.6  & 4.0
\end{tabular}
\caption{ Regression performance on first-order Theory of Mind uncertainty quantification (1TUQ). No BoT or demographic data is used. Direct forecasts (\texttt{DF}) are linearly correlated ($R=0.14$) before scaling, but only linear post-hoc scaling (\texttt{LS}) calibrates these forecasts to be good predictors ($R^2$ up to $12.5\%$). A slight non-linear, monotone relationship also exists ($\rho = 0.16$), but this is not well-modeled by Platt scaling. Tuning a regression head with 8x more data or about 800 data points (\texttt{xl}) does not explain more variance. With the same data, scaling forecasts offers improvement.}
\label{tab:tuq-1}
\end{table}
%
\begin{table*}[]\centering\small
\begin{tabular}{llllllllll}
\textbf{BoT} & \textbf{DEM} & \texttt{Llama3 8B} & \texttt{Mix 8x7B} & \texttt{Gemma 7B} & \texttt{GPT 3.5} & \texttt{Avg} & \texttt{Llama3 70B} & \texttt{Mix 8x22B} & \texttt{GPT 4o} \\\cmidrule(lr){1-2}\cmidrule(lr){3-7}\cmidrule(lr){8-10}
\xmark      & \xmark           & 0.7      & 1.3        & 0.0        & -0.3  & 0.4 & 0.1       & 2.5         & 2.2  \\
\xmark      & \checkmark          & -1.5     & 0.7        & 0.7    & -1.0  & -0.3 & \textbf{0.7}       & \textbf{3.2}         & \textbf{3.3}  \\\hline
\checkmark     & \xmark           & \textbf{0.8}      & \textbf{1.4}        & \textbf{1.9}    & 0.0    &  1.0 & \xmark            &    \xmark           &     \xmark   \\
\checkmark     & \checkmark          & 0.8      & 0.6        & 0.7    & \textbf{0.6} & 0.7 &  \xmark & \xmark           &    \xmark          
\end{tabular}
\caption{ Explained variance (\%) micro-averaged across CANDOR and CaSiNo for 1TUQ task. Results ablate demographic data (in prompt) and BoT (\S~\ref{sec:b_and_v}). Demographic context (DEM) tends to only help larger model's direct forecasts (LS), while smaller models fail to make use of it. Bagging (BoT) tends to help, or have no effect, on smaller models. At least, it mitigates degradation of $R^2$ when including demographic data.}
\label{tab:tuq-1-ablation}
\end{table*}
%
\begin{table*}[]
\centering\small
\begin{tabular}{llllllllll}
\textbf{Dataset}  & \texttt{Llama3 8B} & \texttt{Mix 8x7B} & \texttt{Gemma 7B} & \texttt{GPT 3.5} & \texttt{Llama3 70B} & \texttt{Mix 8x22B} & \texttt{GPT 4o} & \texttt{Avg}& \texttt{Hum}  \\\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}
\textbf{CANDOR}   & -0.2    & \textbf{2.3}       & 0.2   & 0.1   & -0.4      & \textbf{1.0}          & 0.6 & 0.5 & 2.7 \\
\textbf{CaSiNo}   & 1.7      & 0.5        & \textbf{3.6}   & 0.0       & 0.6       & \textbf{3.9}         & 3.7 & 2.0 & \xmark \\
\textbf{MultiWOZ} & \textbf{4.8}      & 2.6        & 4.4    & 3.3   & 4.5       & 2.8         & \textbf{6.8} & 4.2 & \xmark \\\hline
\textbf{Avg} & 2.1 (0.6) & 1.8 (1.6) & 2.7 (0.7) & 1.1 (0.0) & 1.5 & 2.5 & \textbf{3.7}
\end{tabular}
\caption{Explained variance for direct forecasts (LS) on 1TUQ task separated by data and model. BoT is used for small models. Parentheses show $R^2$ without bagging. Models show varied success on different data, meanwhile BoT improves small models to outperform others 10x larger. \texttt{Hum} denotes human $R^2$, after LS (MAE=17.7).}
\label{tab:tuq-1-datasets}
\end{table*}
%
\begin{table*}[]
\centering\small
\begin{tabular}{llllllllll}
\textbf{BoT} & \textbf{DEM} & \texttt{Llama 3 8B} & \texttt{Mix 8x7B} & \texttt{Gemma 7B} & \texttt{GPT 3.5} & \texttt{Avg} & \texttt{Llama 3 70B} & \texttt{Mix 8x22B} & \texttt{GPT 4o}  \\\cmidrule(lr){1-2}\cmidrule(lr){3-7}\cmidrule(lr){8-10}
\xmark  & \xmark     & -1.4       & -0.9         & -0.7     & -0.4   & -0.9 & 0.4         & 1.0             & 0.1  \\
\xmark  & \checkmark & 0.0          & 1.4          & -0.7     & -0.2  & 0.1  & \textbf{0.7}         & \textbf{1.8}           & \textbf{0.7} \\\hline
\checkmark & \xmark     & \textbf{0.8}        & 0.6          & -1.8     & \textbf{1.8}   & 0.4  &      \xmark       &         \xmark      &    \xmark   \\
\checkmark & \checkmark    & 0.6        & \textbf{1.5}          & \textbf{-0.6}     & -0.3 & 0.3  &    \xmark         &   \xmark            &    \xmark    
\end{tabular}
\caption{Explained variance (\%) for 2TUQ task on CANDOR dataset. As before, bagging (BoT) helps smaller models, sometimes pushing them to perform at the level of their larger counterparts. In second-order ToM UQ, demographic data (DEM) appears to help most models, albeit bagging complicates this result for smaller models.}
\label{tab:tuq-2-ablation}
\end{table*}
%
\begin{table}[]
\centering\small
\begin{tabular}{llllll}
   \texttt{method} & \texttt{xl}    & MAE     & $R^2$     & $\min R^2$ & $\max R^2$ \\\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-6}
\texttt{DF (LS)}  & \xmark    & 24.2 & -0.9 & -2.5  & -0.1   \\\hline
\texttt{DF (LS)}& \checkmark  &   24.3    &  -1.9 & -7.0  & -0.2 \\ 
\texttt{FT (RF)} &\checkmark  &  24.8    &  -5.2 & -8.9  & -2.2 \\
\texttt{FT (RF-J)} &\checkmark  &  23.9    &  0.3 & -1.7  & 1.4
\end{tabular}
\caption{Regression metrics for False Uncertainty prediction (FUnQ) on CANDOR. Even with more data, neither direct forecasting (LS) nor fine-tuning is able to explain variance in the ground-truth false uncertainty. False uncertainty prediction is a more difficult task, requiring models to perspective shift and properly predict both the interlocutor's uncertainty and that of the outside world, accurately and simultaneously.}
\label{tab:funq}
\end{table}
%
\subsection{Setup}
\paragraph{Data \& Seeds} We use the 3 datasets/prompting schemes discussed in \S~\ref{sec:data}. More details on prompts are in \S~\ref{sec:prompts}. We use 5 different random seeds to create 5 distinct train/test splits. For training, $n=100$ unless otherwise noted.
\paragraph{Models} Direct forecasting (\texttt{DF}) is conducted with \texttt{Llama3 8B} and \texttt{70B} \citep{llama3modelcard}, \texttt{Mixtral 8x7B} and \texttt{x22B} (v0.1 \citealp{jiang2024mixtral}), \texttt{Gemma 7B} \citep{gemmateam2024gemma}, \texttt{GPT 3.5} (turbo-0125, OpenAI) and \texttt{GPT-4o} (2024-05-13, OpenAI). All models are instruction-tuned (chat) versions. We use default sampling parameters, given on the API or model repository. For fine-tuning (\texttt{FT}), we use latent representations from a pre-trained masked language model, specifically fine-tuned for long-context embedding (M2-BERT, \citealp{fu2024monarch}), which regularly beats much larger models at embedding tasks \citep{monarch}. We use Together AI and Open AI APIs for inference.  
\paragraph{Metrics} We report standard regression metrics including the Pearson (linear) correlation $R$, the Spearman (rank) correlation $\rho$, the mean absolute error $\mathrm{MAE}$, and the \% of variance in the test data explained by the predictions $R^2$. Explaining more variance is better, but it's not typical to explain all of it ($R^2 = 100\%$). For reference, 
%experimental manipulations in psychological studies explain up to 40\% variance in the dependent variable, on average \citep{smedslund2022psychological}. Meanwhile, 
explained variance in (traditional) forecasting tasks with language models is low (up to 10\% Brier Skill Score -- a type of explained variance for soft classifiers, \citealp{sicilia2024deal}). Generally, we use train data to compute the mean when estimating variance on the test set (called ``out-of-sample'' $R^2$ ), which provides a fair evaluation on held-out sets. In this context, $R^2$ can also be interpreted as percent improvement compared to a constant mean prediction. For $\mathrm{MAE}$, we report the \textit{additive} error in \% probability (e.g., $\lvert 0.2 - 0.4 \rvert \times 100\% = 20\%$). Finally, metrics are micro-averaged over all data splits.
\subsection{Results \& Analysis}
We structure our results using a research question (RQ) / answer (A) format, with detailed discussion following each.
\begin{displayquote}
\textit{RQ1: Can language model's predict the uncertainty of other interlocutors in a conversation?} \\
\textit{A: No. Inference ``out-of-the-box'' is poor, but some post-hoc scaling methods enable better prediction.}
\end{displayquote}
\paragraph{Comparison of Scaling Methods}
Table~\ref{tab:tuq-1} reports regression metrics for first-order ToM UQ (1TUQ) split according to different methods of inference. While direct forecasts are ineffective ``out-of-the-box,'' linear scaling (\texttt{DF} \texttt{LS}) with 100 data points can improve scores to a positive explained variance, on average. These results suggest a consistent (if slight) linear relationship between the language model's inferences and the interlocutors' true uncertainty. Explained variance sometimes exceeds 7\%, or with more data, 12\%. Contrary to conventional wisdom (using soft classifiers to forecast outcomes), a logit-linear relationship between the model's inferences and it's target seems unlikely, due to the poor performance of \texttt{DF} \texttt{PS}. % will talk
% \paragraph{Potential for Fine-Tuning} Albeit more data intensive (8$\times$), fine-tuning shows promise. Using a random forest trained on a model's latent space does explain variance on average, up to 7.6\%. 
% The limitation of the current approach is the lack of available data. Increased scale has the potential to allow language models to be fine-tuned to improve their inference about mental states that are represented on a spectrum.
\begin{displayquote}
\textit{RQ2: Does variance reduction via bagging improve language model capability at our regression task?} \\
\textit{A: Yes. Random forests trained on language model embeddings show promise. The proposed Bag of Thoughts (BoT) strategy also improves inference.}
\end{displayquote}
\paragraph{Variance Reduction Strategies} Use of bagging in fine-tuning (i.e., via random forests) did improve performance as anticipated, compared to other tuning strategies. We recall, bagging is a known variance reduction strategy, which can ultimately reduce errors by this mechanism. Another variance reduction strategy we propose is Bag of Thoughts (BoT). Table~\ref{tab:tuq-1-ablation} reports ablation study of BoT for first-order TUQ, limited to CANDOR and CaSiNo. Ablation is also reported for second-order TUQ, limited to CANDOR, in Table~\ref{tab:tuq-2-ablation}. Findings show BoT has positive impact on small models on average, with particular models/setups seeing substantial gain (2\% bump for \texttt{Gemma 7B} on 1TUQ, more for \texttt{GPT 3.5} on 2TUQ). Performance is amplified more so in Table~\ref{tab:tuq-1-datasets} (includes MultiWOZ). Averaged across all 1TUQ data, BoT allows small models to surpass some large models (particularly, \texttt{Llama3 70B}). We did not try BoT for large models, as their lower throughput (tokens/second) made repeated sampling time consuming. Comparison between BoT and greedy decoding is in Table~\ref{tab:mce_v_temp}.
\paragraph{Why BoT Works} Because we use BoT on direct forecasts, and \textit{then} scale them, BoT actually reduces variance in the feature space of the linear scaling function (not necessarily the predictions). Indeed, comparing before/after BoT shows an increase in the standard deviation of the prediction (+0.5\% proba.). Meanwhile, in feature space (the pre-scaled forecast), the STD decreases by 1.5\% probability. Our hypothesis is that variance reduction in feature space (by BoT) actually increases the signal-to-noise-ratio, mitigating the effects of outlier inferences from the model. Increase correlation between pre-scaled forecasts and ground-truth after applying BoT (+0.03) may confirm this.
\begin{displayquote}
\textit{RQ3: Can interlocutor demographic information be used by an LM to improve ToM UQ?} \\
\textit{A: Yes, depending on model size. Larger models show more consistent ability to use demographic context.}
\end{displayquote}
\paragraph{Use of Demographic Context}
In Table~\ref{tab:tuq-1-ablation} we ablate the role of including demographic data in the prompt (\textbf{DEM}), limited to first-order TUQ on CANDOR and CaSiNo. With or without BoT, adding demographics tends to hurt performance of small models (0.7\% and 0.4\% drop in average $R^2$, respectively). Meanwhile, the scaled inferences of larger models are all improved by including demographics. 
%Model size is known factor in language model inference \citep{x}, and may also play a role here, allowing larger models to properly represent the statistical trends evoked by included background information, and preventing smaller models from seeing similar performance boosts. 
In similar ablation for second-order TUQ (Table~\ref{tab:tuq-2-ablation}), we did find less conclusive evidence of a distinction between smaller and larger models use of demographic context. Without BoT, demographics seem to help both small/large models, but with BoT smaller models show mixed responses. 
\paragraph{Demographics and Bias}
Our initial hypothesis was the bias reduction was the principle mechanism by which demographic context could reduce error. This is consistent (for large models, 1TUQ) with observed reduction in bias after including demographics (-0.1\%). The limited effect size does suggest potential for other factors. For instance, similar to variance reduction, interplay between demographic data and scaling may play a role. On the other hand, models (in general) may be ineffective in using demographic context.
% \paragraph{Model Comparison} Table~\ref{tab:tuq-1-datasets} reports explained variance for 1TUQ for \texttt{DF LS}, split by model and dataset. \texttt{GPT-4o} and \texttt{Mix 8x22B} offer the best performance with \texttt{GPT} beating out \texttt{Mixtral} for first place, primarily on MultiWOZ. Interestingly, \texttt{Gemma 7B} (with BoT) outperforms two of the larger models, on average. The performance of \texttt{Llama3} \texttt{70B} was also surprising, as it is often improved by much smaller models (if they use BoT). Table~\ref{tab:tuq-2-ablation} also reports explained variance, split by model, for 2TUQ. Here, \texttt{Gemma} does not perform as well and neither does \texttt{GPT-4o} (i.e., the fair comparison across tables is \textit{without} demographic data). The most successful models are the \texttt{Mixtral} models, suggesting a unique advantage from their training data (closed-source) or their MoE architectures. \texttt{GPT 3.5} also shows promise in 2TUQ, under one setting (BoT, no demographics), but is less robust to perturbations among settings.
\begin{displayquote}
\textit{RQ4: What factors of conversation context and ToM task impact LM inferences about uncertainty?} \\
\textit{A: Longer conversations are more difficult for LMs. Humans may also hide goals in some contexts (e.g., negotiation), compounding difficulty. LMs also show difficulty when shifting perspectives.}
\end{displayquote}
\paragraph{Data Comparison} 
% Returning to Table~\ref{tab:tuq-1-datasets},
Table~\ref{tab:tuq-1-datasets} reports explained variance for 1TUQ for \texttt{DF LS}, split by model and dataset. We observe CANDOR to be the most difficult dataset for 1TUQ, followed by CaSiNo, then MultiWOZ. One hypothesis for the difficulty of CANDOR is the length of it's conversations, which average more than 11K tokens (GPT-2 tokenizer). This may also be compounded because dialogue is between strangers. Small, but important, nuances can become dominated other -- perhaps, superficially polite -- interactions. The reality that humans can hide their true mental states may also explain increased difficulty in CaSiNo, a negotiation corpus. Rather than ``acting'' to be polite, interlocutors in the CaSiNo corpus hide motives and intentions, as a strategy, to receive a better deal. In contrast, in the collaborative and task-oriented MultiWOZ corpus, interlocutors have incentive to reveal many aspects of their mental state; e.g., to indicate satisfactory constraints for their booking task. 
% Satisfaction of these goals may be inferred from conversation, making it easier to predict the uncertainty of this mental state.
\paragraph{Task Comparison} Our methods are effective for (at least some models) on both first-order and second-order TUQ. We refrain from commenting on the differences in difficulty between these, since it varies widely depending on model. The task that stood our was False Uncertainty Quantification (FUnQ), which has results split by method in Table~\ref{tab:funq}. The key observation is that, unlike previous tasks, no model achieves positive explained variance via direct forecasting, even after scaling. This is evidenced by the negative maximum $R^2$ value. The best fine-tuning strategies offer some improvement, but performance is still relatively low.
\paragraph{Why FUnQ is Hard}
We hypothesize this difficulty may, in part, come because model errors compound across multiple inference steps; e.g., the inference for interlocutor's uncertainty $\hat{P}$ and the inference for the ground-truth probability $\hat{p}$. Indeed, one data point in favor of this hypothesis is the positive explained variance of the joint fine-tuning procedure (\texttt{FT} \texttt{RF-J}), which conducts non-linear inference over the embedding of both prompts (i.e., to infer $\hat{P}$ and $\hat{p}$) and then produces a single estimate for the difference $P - p$. 
% Other methods which use prompt structure to have models directly forecast this difference will be of future interest, but it's not clear how to best extract this information from the model, as of yet. On the other hand, the datasets we work with are still relatively small, even for fine-tuning (recall, about 800 training points). Increased data for fine-tuning can help models learn more well-defined statistical trends between interlocutor beliefs and the subjects of these beliefs to better quantify false uncertainty.
\begin{displayquote}
    \textit{RQ5: How do humans perform at ToM UQ tasks?} \\
    \textit{A: Slightly better than LMs (scaling is still needed).}
\end{displayquote}
\paragraph{Human Performance} Because of available annotations (\S~\ref{sec:data}), we infer human performance at first-order ToM UQ on CANDOR. Interestingly, linear scaling also improves the performance for human forecasts, which may be suggestive of individual baselines for how people express their uncertainty (or, intensity) about beliefs. Human performance is not drastically higher than models ($R^2=2.7\%$, MAE=17.7), which is again suggestive of the difficulty of this corpus (recall, our data comparison).
\begin{displayquote}
    \textit{RQ6: Can uncertainty estimates improve LM inference at routine ToM (i.e., belief classification)?} \\
    \textit{A: Yes. In \S~\ref{sec:case_study}, we conduct a case-study with Llama 3 and CaSiNo. Using uncertainty estimates to infer beliefs improves accuracy and F1 score.}
\end{displayquote}
%: one person's 4/7 is not necessarily another's. Although, this may also be suggestive of the difficulty of the task on this corpus. Indeed, explained variance (with linear scaling) is only 2.7\% with MAE = 17.7\% probability. As noted, difficulties can arise from the nuances of a first meeting, especially as these are situated in the context of a much larger interaction. While demographic information can be inferred by human interlocutors (visually), there is plenty of additional background information / context that is unavailable to strangers meeting for the first time (i.e., which also makes the situation similar to a model viewing two interlocutors for the first time). In this sense, it is somewhat unsurprising that a fine-grained representation of another's mental states is not easily inferred (even by humans) from a first-time encounter. Future research might consider ToM UQ given repeated interactions and how this long-term context can be represented to improve performance.  
% \paragraph{First-Order Theory of Mind UQ}
% Table~\ref{tab:} reports regression metrics for 1TUQ split by methods and averaged over data/splits. Findings include:
% \begin{itemize}[nolistsep]
%     \item most methods have about 20\% MAE, so uncertainty estimates are off by 0.2 on average;
%     \item ``out-of-the-box'' direct forecasting (\texttt{DF}) fails to explain any variation in the test data, except when forecasts are linearly scaled (Eq.~\ref{eqn:x})
%     \item fine-tuning is ineffective except with more data and bagging methods (random forests), in which case \texttt{DF} \texttt{(LS)} improves as well.
% \end{itemize}
% %
% \paragraph{Ablation Study and 2TUQ}
% Table~\ref{tab:} reports ablation study of Monte Carlo Estimation (\textbf{BoT}) and Demographics (\textbf{DEM}) for 1TUQ using \texttt{DF} with linear scaling on CANDOR and CaSiNo. We report explained variance for \texttt{DF} with linear scaling, since other methods remained ineffective, and report metrics split by model. Table~\ref{sec:} reports the same ablation study for Second-Order Theory of Mind UQ (2TUQ) on the CANDOR dataset. Important findings from these tables include:
% \begin{itemize}[nolistsep]
%     \item larger models consistently make use of demographic data in the prompt to improve predictions, while smaller models are inconsistent;
%     \item BoT consistently improves small models, enabling some scores to surpass larger models.
% \end{itemize}
% \paragraph{Data \& Model Comparison}
% Table~\ref{tab:} reports explained variance for 1TUQ for \texttt{DF} with linear scaling, split by model, for all datasets:
% \begin{itemize}[nolistsep]
%     \item CANDOR is the most difficult dataset for 1TUQ, followed by CaSiNo, then MultiWOZ;
%     \item BoT offers even more improvement when including MultiWOZ in the average $R^2$, allowing most small models to beat \texttt{Llama3 70B} as well as rival other large models;
%     \item \texttt{GPT-4o} and \texttt{Mixtral 8x22B} offer the best performance with \texttt{GPT} beating out \texttt{Mixtral} for first place, primarily on MultiWOZ;
%     \item human (\texttt{Hum}) performance (with linear scaling) is available for CANDOR only, and surpasses all models.
% \end{itemize}
% \paragraph{False Uncertainty Quantification}
% Finally, Table~\ref{sec:} reports performance, split by method, for False Uncertainty Quantification (FUnQ). No methods enable explanation of variance by language models on this task. 
% \subsection{Discussion}
% \paragraph{A Modest Linear Relationship} The methods we use to extract uncertainty forecasts from language models tend to have seemingly modest performance, but we do find that simple linear scaling of the LM inference offers a consistently effective, low-resource strategy (uses 100 data points). Test error may seem high (20\% proba.) with limited explained variance ($\leq$ 8\%), but these (modest) results are consistent with other use of language models for forecasting in conversational settings. For instance, \citep{sicilia} observe many language models explain similar magnitude of variance in traditional forecasting on negotiation corpora; they report Brier skill score, an adaptation of $R^2$ for the hard outcome annotations. More data or improved models may abate concerns, but high scores (e.g., $R^2 = 90\%$) are rare for experiments involving humans: a study of the psychology literature found independent (manipulated) variables explained about 43\% variance, averaged across studies \citep{x}. Even linear scaling of human inferences (Table~\ref{tab:}) offers only 2.7\% explained variance ($R=0.2$, MAE=$17.7$). 
% \paragraph{Fine-tuning has Potential} Non-linear methods operating on model latent space may offer a future avenue of success, as indicated by the somewhat promising results
% \paragraph{How Models Use Demographics}
% % bias is reduced in magnitude by .1% probability on average
% \paragraph{How BoT Improves Performance}
% % variance is not perceptibly decreased (to 3 significant digits), but bias shows a similiar relationship to demographics
% % std increases by about 0.005 for yhat
% % decreases by about 0.014 in the feature
% % so the reduces variance in the feature helps the scaling reduce bias, rather than reducing variance of prediction directly
% % correlation also goes up 0.125 to 0.152
% % overall, we are averaging out noise in the feature 
% \paragraph{How Context Length Impacts Performance}
% \paragraph{How Hidden Motives Impact Performance}
% \paragraph{Models Fail to Predict False Uncertainty}

==> 05_concl.tex <==
This paper details tasks and methods to explore how language models represent the uncertainty of other interlocutors in conversations. We make connections between this task and Theory of Mind, suggesting a continuous analog of false beliefs (we call, false uncertainty) and asking models to quantify it. High-level findings are summarized below:
\begin{itemize}[nolistsep]
    \item language models can explain variance in others' uncertainty on some corpora (up to 7\%), but humans may hide mental states in social dialogue and negotiations;
    \item humans themselves can have trouble with this task (in social dialogue) and appear to have different baselines for the intensity of their beliefs;
    \item variance and bias reduction are important mechanisms for tailoring language models to regression tasks;
    \item perspective shift in uncertainty modeling is difficult, as language models experience compounding errors that prevent accurate prediction of false uncertainty.
\end{itemize}
We also highlight some areas of future work.
\paragraph{Dialogue Policy and Generation} A motivation of our work is machine dialogue, as recognizing false uncertainty can inform dialogue acts, like explanation, as well as how to execute such an act. Prior work uses ToM to directly inform dialogue policies and generation \citep{zhou-etal-2023-cast}, and our ToM UQ methods may be fruitful in such contexts.
\paragraph{Communication Theories} Accurate and automated quantification of uncertainty in interlocutors has the potential to scale up studies of uncertainty in communication, and communication theories founded on uncertainty \citep{berger1974some, sunnafrank1986predicted} to large corpora. For instance, in data driven studies of these theories, participant annotation of uncertainty is needed \citep{yoo2009uncertainty}, but may be relaxed with suitable automated methods. The role of uncertainty in alternate communicative theories, such as grounding \citep{clark1991grounding} is also of interest.
\paragraph{Demographics and Uncertainty} Our methodological findings -- that demographics can improve inference about others' uncertainty -- suggest these factors may play an important role in how individuals express and manage uncertainty. Further study of this connection can prevent unintended biases in the dialogue systems we create.
\paragraph{Methodology} We leave ample room for improvement on these ToM UQ tasks. While fine-tuning showed potential in our results, the scale of available data was a limiting factor. Work-arounds, e.g., simulation, can enable full model fine-tuning, as in previous forecasting work \citep{sicilia2024deal}. False uncertainty quantification, in particular, may benefit from new methodologies which can improve models' ability to shift perspectives -- a more broadly useful capability; e.g., for LLM-based agent simulations \citep{park2023generative}.
\section*{Acknowledgements} This research was supported in part by Other Transaction award HR0011249XXX from the U.S. Defense Advanced Research Projects Agency (DARPA) Friction for Accountability in Conversational Transactions (FACT) program. Thanks to Mert Inan for helpful feedback.
% \section*{Limitations}
% As noted in our conclusions, there are many aspects of this research which call for continued development. For instance, we study relatively simple fine-tuning strategies and do not explore downstream applications directly in our experiments. The purpose of this work is to propose an evaluation methodology and some initial algorithms. We acknowledge the limited scope of our initial experiments, with respect to these topics of future work.

% Moreover, while we do study three diverse corpora, generalization of our findings to new data is not guaranteed. Different outcomes or corpora may show worse results from the studied language models. Scientific conclusions drawn about this data may not generalize to new corpora either. Reproducibility studies and greater data collection is needed to allow the tasks we propose to be studied at a larger scale, to mitigate concerns about generalization of methods/findings.

% While we do motivate this work from the point-of-view of ToM, we do recall some potential caveats we brought up when outlining ToM evaluation criteria (\textbf{ToM Criteria}). Namely, our setup does not explicitly control for potential spurious correlations between the dialogues we use as features and the target predictions we evaluate as a proxy for ToM capability. For this reason, one should be careful to interpret our results as suggesting language models have (any level) of ToM capability. With that said, future research can incorporate more data controls (without changing our task designs) to help mitigate any present limitations from the corpora we study. It should also be noted that it is not clear whether ToM is a capability that can ever truly exist in language models, at least in a human sense. Exactly what counts as ``reasoning'' about human's mental states and what is purely ``statistical parrot''-like behavior is a topic of debate, which this paper does not aim to address. Simply, we aim to propose tasks that can evaluate (or, approach evaluation) of abilities traditionally associated with ToM in humans.  

% Finally, there are many other aspects of ToM, besides anticipation of beliefs and false beliefs, which we do not cover in this paper. Some of the mentioned works in our paragraph \textbf{Other ToM Works} include study of other sub-topics, under the broad umbrella of ToM. We focus on false beliefs because of the practical value that considering uncertainty of beliefs can have.
% \section*{Ethics}
% The data we use in this study is either publicly available or available at the request of the respective dataset authors. Our use of this data is consistent with any license or terms of use attached to the data. Some of the data used in this study may contain personally identifying information. Appropriate care should be taken, whenever re-creating our evaluation setup, about the consequences of this fact.  Details on these and other ethical considerations are discussed by the datasets original authors.

% The models we study, and therefore methods we propose (built on these models), may have social biases inherited from their training data. Although bias mitigation and other safety protocols can be put in place to mitigate concerns, using these models can also introduce (unexpected) biases however they are deployed. For instance, if used in the applications we suggest, they might change a dialogue systems policy, and this change could disproportionately impact a subset of users. The scale of impact is made greater by the ability to use our methods without much human supervision. Thus, deployment of these models should consider the potential impact on users and other far-reaching consequences that improperly moderated use of our models can create.

==> 08_repro_checklist.tex <==
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes}/partial/no/NA)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{yes}/no)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{yes}/no) 
\end{itemize}

Does this paper make theoretical contributions? (yes/\textbf{no})

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

Does this paper rely on one or more datasets? (\textbf{yes}/no)

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\textbf{yes}/partial/no/NA)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/\textbf{NA})
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\textbf{NA})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textbf{yes}/no/NA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textbf{yes}/partial/no/NA)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\textbf{NA})
\end{itemize}

Does this paper include computational experiments? (\textbf{yes}/no)

If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (\textbf{yes}/partial/no).
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{yes}/partial/no)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes}/partial/no)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{yes}/partial/no)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{yes}/partial/no/NA)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{yes}/partial/no)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes}/partial/no)
    \item This paper states the number of algorithm runs used to compute each reported result. (\textbf{yes}/no)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{yes}/no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/\textbf{no})
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{yes}/partial/no/NA)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{yes}/partial/no/NA)
\end{itemize}









